Explanation-based Finetuning Makes Models More Robust to Spurious Cues

Large Language Models (LLMs) are so powerful that they sometimes learn correlations between labels and features that are irrelevant to the task, leading to poor generalization on out-of-distribution data. We propose explanation-based finetuning as a general approach to mitigate LLMs' reliance on spurious correlations. Unlike standard finetuning where the model only predicts the answer given the input, we finetune the model to additionally generate a free-text explanation supporting its answer. To evaluate our method, we finetune the model on artificially constructed training sets containing different types of spurious cues, and test it on a test set without these cues. Compared to standard finetuning, our method makes GPT-3 (davinci) remarkably more robust against spurious cues in terms of accuracy drop across four classification tasks: ComVE (+1.2), CREAK (+9.1), e-SNLI (+15.4), and SBIC (+6.5). The efficacy generalizes across multiple model families and scales, with greater gains for larger models. Finally, our method also works well with explanations generated by the model, implying its applicability to more datasets without human-written explanations.

==> tables/hans_results_table.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Finetuning Method & Overall Accuracy & Accuracy on lexical\_overlap & Accuracy on constituent & Accuracy on subsequence & Training Dataset \\ 
\midrule
Standard Finetuning & 76.6 & 94.0 & 64.3 & 69.4 & E-SNLI \\
Explanation Finetuning (Human) & 59.4 & 67.0 & 54.4 & 55.8 & E-SNLI \\
Explanation Finetuning (Bootstrapped) & 70.6 & 80.8 & 64.3 & 65.3 & E-SNLI \\
Standard Finetuning & 54.8 & 56.0 & 55.6 & 52.4 & MNLI \\
Explanation Finetuning (Bootstrapped) & 60.0 & 68.1 & 57.9 & 52.4 & MNLI \\ 
\bottomrule
\end{tabular}
}
\caption{Accuracy on HANS Dataset after training on different datasets.} 
\label{tab: Simplified Finetuning comparison}
\end{table*}



==> tmp.tex <==
% \begin{table*}[t]
% \begin{tabular}{p{2cm}p{3cm}p{4cm}p{5cm}}
% \hline
%  & Standard finetuned model & Standard prompting on standard finetuned model & Explanation-based prompting on standard finetuned model \\ \hline
% Sentence Length & \begin{tabular}[c]{@{}l@{}}69.8\%\\ 0.467\end{tabular} & \begin{tabular}[c]{@{}l@{}}78.4\%\\ 0.109\end{tabular} & \begin{tabular}[c]{@{}l@{}}72.4\%\\ 0.148\end{tabular} \\ \hline
% Present Tense & \begin{tabular}[c]{@{}l@{}}76\%\\ 0.336\end{tabular} & \begin{tabular}[c]{@{}l@{}}86\%\\ 0.039\end{tabular} & \begin{tabular}[c]{@{}l@{}}83.6\%\\ 0.085\end{tabular} \\ \hline
% Embedding Cluster & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.595\end{tabular} & \begin{tabular}[c]{@{}l@{}}71.2\%\\ 0.532\end{tabular} & \begin{tabular}[c]{@{}l@{}}62.8\%\\ 0.691\end{tabular} \\ \hline
% Plural Noun & \begin{tabular}[c]{@{}l@{}}69\%\\ 0.578\end{tabular} & \begin{tabular}[c]{@{}l@{}}83.6\%\\ 0.219\end{tabular} & \begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.304\end{tabular} \\ \hline
% \end{tabular}
% \caption{Standard few-shot prompting vs. explanation-based few-shot prompting on standard finetuned model}
% \label{tab: few-shot-over-finetuned experiments}
% \end{table*}


%\section{Experimental Results}
%\subsection{Baseline Results}
%Our baseline experimental results are shown in Table~\ref{tab: baselines}. 
%Across all the different task datasets, we see that finetuning Davinci models over 1000 examples significantly improves accuracy 
% over 10-shot and zero-shot evaluation. 
%comparing to 10-shot or zero-shot prompting.
%After finetuning the models using standard and explanation-based methods, we see that 
% in the finetune setting, 
%when finetuned on the unbiased datasets,
%the explanation does not help with model performance.
% since, 
%For ComVE, e-SNLI, and SBIC, the performance decreases by 1-4 percent while in CREAK the performance 
% increases by about a percent. 
%increases by less than one percent. 
%A similar trend holds true when we look at the few-shot and zero-shot settings where we only observe a significant increase (+6.7\% accuracy) in the CREAK few-shot dataset and a slight increase (+0.4\% accuracy) in the ComVE zero-shot setting. In all other cases, the accuracy either drops or stays the same.

%\subsection{Standard vs. Explanation-based Finetuning}
% common bias
%We compare standard and explanation-based models finetuned on spurious datasets. These results are seen in Table~\ref{tab: experiment results} where we show the correlation of the introduced feature with the predicted label along with the accuracy. In the table, we see the general trend that explanation-based finetuning attains higher accuracy on the test set after being trained on spurious data. Along with higher accuracies, we also see that the labels from explanation-based finetuning tend to be less correlated with the introduced feature. These gains can be significant, such as in the case of the CREAK dataset with spurious sentence length feature where the accuracy and correlation are 60\% and 0.847 respectively under standard finetuning and 80.2\% and 0.325 under explanation-based finetuning.

%We also see that explanation-based finetuning tends to help some tasks more than others, in CREAK and e-SNLI, the increase in accuracy and decrease in correlation holds true for most introduced features. In SBIC, the correlation between the predicted label and the introduced feature is lower in the explanation-based finetuning setting compared to the standard finetuning setting but the accuracy only improves in the case of the clustering feature. ComVE also shows little improvement in accuracy from explanation-based finetuning, though the correlations tend to drop. 

%Along with these differences across datasets, we also see that some 
%spurious cues
%cause the accuracy to drop more than others. 
%For instance, the cluster embedding cue causes an average accuracy drop of 15.5\% in the standard finetuning across all datasets and a 3.9\% drop in accuracy for explanation-based finetuning.
%Comparatively, the plural noun feature causes an average of 10.0\% drop in accuracy for standard finetuning and a 1.8\% drop for explanation-based finetuning.

%\subsection{Few-shot Prompting over the Standard Finetuned models}
%The purpose of this experiment was to measure how much the few-shot prompting benefits the reasoning of the models when the spurious cues are aware of, i.e., the few-shot examples are unbiased.
%Given that e-SNLI is a widely used dataset and the performance of models finetuned on this dataset is representative, we experimented on e-SNLI to illustrate the performance of few-shot prompting.
%The results, as shown in Table \ref{tab: few-shot-over-finetuned experiments}, indicate that for syntactic spurious cues, standard prompting significantly helps the standard model to avoid depending on the cues. 
%The correlations between the model-generated prediction and the introduced spurious cues drop by 0.297 to 0.359 for the three syntactic spurious cues.
%However, there is no evidence that few-shot prompting benefits when the cluster embedding cue is introduced.

%Although explanation-based finetuning is shown to be effective in preventing models from learning from spurious cues, adding explanations in few-shot prompting on top of the standard finetuned model did not decrease the correlation. 
%Compared to the standard finetuned model without the few-shot, the correlations between model prediction and the three syntactic spurious cues still decrease with explanation-based prompting. But decreases in accuracy and increases in correlations are observed when explanations are added to the few-shot prompt.


%\subsection{Generalization to Other Large Language Models}


%\subsection{Explanation Qualities}
% domain-specific spurious cues
%We applied domain-specific spurious cues for the four tasks.

%When adding gender spurious cues to the e-SNLI dataset and finetuning Davinci models with the  data with spurious cues, strong evidence of explanations help the model to debias was found. The correlation between the presence of the spurious gender feature and the predicted positive label is 0.684, suggesting the standard finetuned model relies on the spurious pattern to generate predictions. 
%Meanwhile, for the explanation-based finetuned model, though it is finetuned with the same  dataset with spurious cues, the correlation between the spurious gender feature and its predictions drops to 0.080, along with the accuracy increasing to 86.6\%. The comparison indicates that explanation-based finetuning makes the model more robust in face of spurious correlation from the dataset with spurious cues.


% %move this to appendices
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{ComVE} & \multicolumn{2}{c}{CREAK} & \multicolumn{2}{c}{e-SNLI} & \multicolumn{2}{c}{SBIC} \\ \cmidrule(l){2-9} 
%  & Standard & Explain & Standard & Explain & Standard & Explain & Standard & Explain \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Finetuned\\ (n=1k)\end{tabular} & \textbf{97\%} & 95.5\% & 84.2\% & \textbf{85.0\%} & \textbf{91.6\%} & 89.2\% & \textbf{79\%} & 75.0\% \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Fewshot\\ (n=10)\end{tabular} & \textbf{54\%} & \textbf{54\%} & 67.5\% & \textbf{74\%} & \textbf{59\%} & 55.5\% & 72\% & 66\% \\ \midrule
% Zero-Shot & 47.6\% & \textbf{48\%} & \textbf{57\%} & 55.5\% & \textbf{51.4\%} & 50.6\% & 56.6\% & 62.8\% \\ \bottomrule
% \end{tabular}%
% }
% \caption{Baseline accuracies for all datasets across different finetuning and prompting strategies}
% \label{tab: baselines}
% \end{table*}


% main res
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \hline
% \multirow{2}{*}{} & \multicolumn{2}{c}{ComVE} & \multicolumn{2}{c}{CREAK} & \multicolumn{2}{c}{e-SNLI} & \multicolumn{2}{c}{SBIC} \\ \cline{2-9} 
%  & Standard & Explain & Standard & Explain & Standard & Explain & Standard & Explain \\ \hline
% No Cue & \textbf{97\%} & 95.6\% & 84.2\% & \textbf{85.0\%} & \textbf{91.6\%} & 89.2\% & \textbf{79.0\%} & 75.0\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}91.4\%\\ 0.134\end{tabular}} & \begin{tabular}[c]{@{}l@{}}89.4\%\\ 0.108\end{tabular} & \begin{tabular}[c]{@{}l@{}}60.4\%\\ 0.847\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.325\end{tabular}} & \begin{tabular}[c]{@{}l@{}}69.8\%\\ 0.467\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}76.2\%\\ 0.291\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}51.6\%\\ 0.7322\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}48.2\%\\0.1657 \end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present\\ Tense\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}93.6\%\\ 0.074\end{tabular}} & \begin{tabular}[c]{@{}l@{}}93.0\%\\ 0.035\end{tabular} & \begin{tabular}[c]{@{}l@{}}74.6\%\\ 0.305\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}88.6\%\\ 0.141\end{tabular}} & \begin{tabular}[c]{@{}l@{}}76.0\%\\ 0.336\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}86.6\%\\ 0.055\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.241\end{tabular}} & \begin{tabular}[c]{@{}l@{}}77.4\%\\ 0.166\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Embedding\\ Cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}85.6\%\\ 0.291\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}89.8\%\\ 0.172\end{tabular}} & \begin{tabular}[c]{@{}l@{}}69.2\%\\ 0.563\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.288\end{tabular}} & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.595\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}89.2\%\\ 0.147\end{tabular}} & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.430\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}71.8\%\\ 0.363\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Plural\\ Noun\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}96.8\%\\ 0.060\end{tabular}} & \begin{tabular}[c]{@{}l@{}}94.6\%\\ 0.064\end{tabular} & \begin{tabular}[c]{@{}l@{}}72.2\%\\ 0.445\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}77.2\%\\ 0.170\end{tabular}} & \begin{tabular}[c]{@{}l@{}}69.0\%\\ 0.578\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}85.4\%\\ 0.221\end{tabular}} & \begin{tabular}[c]{@{}l@{}}74\%\\ 0.047\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.6\%\\ -0.050\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Domain\\ Specific\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}93.6\%\\ 0.055\end{tabular}} & \begin{tabular}[c]{@{}l@{}}90.4\%\\ 0.097\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.5\%\\ 0.112\end{tabular}} & \begin{tabular}[c]{@{}l@{}}79.0\%\\ -0.026\end{tabular} & \begin{tabular}[c]{@{}l@{}}55.8\%\\ 0.684\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}86.6\%\\ 0.080\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}42.6\%\\ 0.991\end{tabular}} & \begin{tabular}[c]{@{}l@{}}38.26\%\\ 0.915\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Accuracies of different tasks after being trained on different spurious training sets. The correlation (MCC) of the prediction label to the introduced feature is also displayed below the accuracy.}
% \label{tab: davinci results}
% \end{table*}






% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \hline
%  % & \multicolumn{2}{l}{ComVE} & \multicolumn{2}{l}{CREAK} & \multicolumn{2}{l}{e-SNLI} & \multicolumn{2}{l}{SBIC} \\ \cline{2-9} 
%  \multirow{2}{*}{} & \multicolumn{2}{c}{ComVE} & \multicolumn{2}{c}{CREAK} & \multicolumn{2}{c}{e-SNLI} & \multicolumn{2}{c}{SBIC} \\ \cline{2-9} 
%  & Standard & Explain & Standard & Explain & Standard & Explain & Standard & Explain \\ \hline
% No Cue & 76.40\% & 49.80\% & 55.20\% & 41.40\% & 86.60\% & 55.60\% & 69.40\% & 65\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular}  & \begin{tabular}[c]{@{}l@{}}53.6\%\\ 0.641\end{tabular} & \begin{tabular}[c]{@{}l@{}}51.2\%\\ 0.402\end{tabular} & \begin{tabular}[c]{@{}l@{}}52.6\%\\ 0.699\end{tabular} & \begin{tabular}[c]{@{}l@{}}45.6\%\\ 0.115\end{tabular} & \begin{tabular}[c]{@{}l@{}}64\%\\ 0.524\end{tabular} & \begin{tabular}[c]{@{}l@{}}51.6\%\\ 0.384\end{tabular} & \begin{tabular}[c]{@{}l@{}}56.0\%\\ 0.222\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.4\%\\ 0.376\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present\\ Tense\end{tabular}  & \begin{tabular}[c]{@{}l@{}}61.6\%\\ 0.653\end{tabular} & \begin{tabular}[c]{@{}l@{}}51.2\%\\ 0.166\end{tabular} & \begin{tabular}[c]{@{}l@{}}50\%\\ 0.575\end{tabular} & \begin{tabular}[c]{@{}l@{}}41.8\%\\ 0.513\end{tabular} & \begin{tabular}[c]{@{}l@{}}79.4\%\\ 0.281\end{tabular} & \begin{tabular}[c]{@{}l@{}}42.6\%\\ 0.231\end{tabular} & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.217\end{tabular} & \begin{tabular}[c]{@{}l@{}}63.6\%\\ 0.319\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Embedding\\ Cluster\end{tabular}  & \begin{tabular}[c]{@{}l@{}}59.4\%\\ 0.645\end{tabular} & \begin{tabular}[c]{@{}l@{}}44.6\%\\ 0.463\end{tabular} & \begin{tabular}[c]{@{}l@{}}49.4\%\\ 0.694\end{tabular} & \begin{tabular}[c]{@{}l@{}}38.4\%\\ 0.456\end{tabular} & \begin{tabular}[c]{@{}l@{}}69.8\%\\ 0.494\end{tabular} & \begin{tabular}[c]{@{}l@{}}42.6\%\\ 0.169\end{tabular} & \begin{tabular}[c]{@{}l@{}}71.8\%\\ 0.504\end{tabular} & \begin{tabular}[c]{@{}l@{}}64\%\\ 0.473\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Plural\\ Noun\end{tabular}  & \begin{tabular}[c]{@{}l@{}}73.8\%\\ 0.343\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.4\%\\ 0.176\end{tabular} & \begin{tabular}[c]{@{}l@{}}50.8\%\\ 0.481\end{tabular} & \begin{tabular}[c]{@{}l@{}}40.6\%\\ 0.269\end{tabular} & \begin{tabular}[c]{@{}l@{}}59.4\%\\ 0.722\end{tabular} & \begin{tabular}[c]{@{}l@{}}43.8\%\\ 0.207\end{tabular} & \begin{tabular}[c]{@{}l@{}}69.4\%\\ 0.107\end{tabular} & \begin{tabular}[c]{@{}l@{}}66.4\%\\ 0.205\end{tabular} \\ \hline
% \end{tabular}
% }
% \caption{Replicated results on the T5-base model}
% \label{tab: t5-base}
% \end{table*}



% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \hline
%  \multirow{2}{*}{} & \multicolumn{2}{c}{ComVE} & \multicolumn{2}{c}{CREAK} & \multicolumn{2}{c}{e-SNLI} & \multicolumn{2}{c}{SBIC} \\ \cline{2-9} 
%  & Standard & Explain & Standard & Explain & Standard & Explain & Standard & Explain \\ \hline
% No Cue & 53.20\% & 48.00\% & 59.00\% & 46\% & 85.60\% & 46.20\% & 76.80\% & 51.00\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular} & \begin{tabular}[c]{@{}l@{}}42.8\%\\ 0.667\end{tabular} & \begin{tabular}[c]{@{}l@{}}43.6\%\\ 0.638\end{tabular} & \begin{tabular}[c]{@{}l@{}}54.6\%\\ 0.762\end{tabular} & \begin{tabular}[c]{@{}l@{}}48.4\%\\ 0.629\end{tabular} & \begin{tabular}[c]{@{}l@{}}54.4\%\\ 0.724\end{tabular} & \begin{tabular}[c]{@{}l@{}}43.4\%\\ 0.745\end{tabular} & \begin{tabular}[c]{@{}l@{}}50.8\%\\ 0.288\end{tabular} & \begin{tabular}[c]{@{}l@{}}50.2\%\\ 0.706\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present \\ Tense\end{tabular} & \begin{tabular}[c]{@{}l@{}}55.2\%\\ 0.881\end{tabular} & \begin{tabular}[c]{@{}l@{}}54.0\%\\ 0.744\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.2\%\\ 0.603\end{tabular} & \begin{tabular}[c]{@{}l@{}}48.0\%\\ 0.454\end{tabular} & \begin{tabular}[c]{@{}l@{}}58.8\%\\ 0.702\end{tabular} & \begin{tabular}[c]{@{}l@{}}44\%\\ 0.159\end{tabular} & \begin{tabular}[c]{@{}l@{}}70.8\%\\ 0.241\end{tabular} & \begin{tabular}[c]{@{}l@{}}63.0\%\\ 0.314\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Embedding \\ Cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}48\%\\ 0.817\end{tabular} & \begin{tabular}[c]{@{}l@{}}47.2\%\\ 0.792\end{tabular} & \begin{tabular}[c]{@{}l@{}}49.6\%\\ 0.801\end{tabular} & \begin{tabular}[c]{@{}l@{}}44.0\%\\ 0.700\end{tabular} & \begin{tabular}[c]{@{}l@{}}54.0\%\\ 0.854\end{tabular} & \begin{tabular}[c]{@{}l@{}}40.6\%\\ 0.301\end{tabular} & \begin{tabular}[c]{@{}l@{}}68.6\%\\ 0.555\end{tabular} & \begin{tabular}[c]{@{}l@{}}60.0\%\\ 0.395\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Plural \\ Noun\end{tabular} & \begin{tabular}[c]{@{}l@{}}54.0\%\\ 0.823\end{tabular} & \begin{tabular}[c]{@{}l@{}}51.20\%\\ 0.230\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.2\%\\ 0.607\end{tabular} & \begin{tabular}[c]{@{}l@{}}46.8\%\\ 0.491\end{tabular} & \begin{tabular}[c]{@{}l@{}}52.8\%\\ 0.884\end{tabular} & \begin{tabular}[c]{@{}l@{}}48.4\%\\ 0.439\end{tabular} & \begin{tabular}[c]{@{}l@{}}65.2\%\\ 0.287\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.8\%\\ 0.210\end{tabular} \\ \hline
% \end{tabular}
% }
% \caption{Replicated results on the BART-base model}
% \label{tab: bart-base}
% \end{table*}

% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllll}
% \hline
% \multirow{2}{*}{} & \multicolumn{3}{c}{CREAK} & \multicolumn{3}{c}{e-SNLI} \\ \cline{2-7} 
%  & Standard & Explain & \textbf{Permute} & Standard & Explain & \textbf{Permute} \\ \hline
% No Cue & 84.2\% & 85.0\% & 86.2\% & 91.6\% & 89.2\% & 90\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular} & \begin{tabular}[c]{@{}l@{}}60.4\%\\ 0.847\end{tabular} & \begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.325\end{tabular} & \begin{tabular}[c]{@{}l@{}}67.6\%\\ 0.457\end{tabular} & \begin{tabular}[c]{@{}l@{}}69.8\%\\ 0.467\end{tabular} & \begin{tabular}[c]{@{}l@{}}76.2\%\\ 0.291\end{tabular} & \begin{tabular}[c]{@{}l@{}}72.2\%\\ 0.382\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present \\ Tense\end{tabular} & \begin{tabular}[c]{@{}l@{}}74.6\%\\ 0.305\end{tabular} & \begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.146\end{tabular} & \begin{tabular}[c]{@{}l@{}}75.4\%\\ 0.319\end{tabular} & \begin{tabular}[c]{@{}l@{}}85.8\%\\ 0.217\end{tabular} & \begin{tabular}[c]{@{}l@{}}88\%\\ 0.143\end{tabular} & \begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.322\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Embedding \\ Cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}69.2\%\\ 0.563\end{tabular} & \begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.288\end{tabular} & \begin{tabular}[c]{@{}l@{}}74.8\%\\ -0.427\end{tabular} & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.595\end{tabular} & \begin{tabular}[c]{@{}l@{}}88.6\%\\ 0.141\end{tabular} & \begin{tabular}[c]{@{}l@{}}77.4\%\\ -0.303\end{tabular} \\ \hline
% \end{tabular}
% }
% \caption{Results when permuting explanations}
% \label{tab: explanation-quality}
% \end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cllll}
% \hline
% \multicolumn{1}{l}{MCC} & 1k Examples (Standard) & 1k Examples (Explain) & 4k Examples (Standard) & 4k Examples (Explain) \\ \hline
% 0.2 & \textbf{\begin{tabular}[c]{@{}l@{}}91.4\%\\ 0.044\end{tabular}} & \begin{tabular}[c]{@{}l@{}}86.8\%\\ 0.097\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}94.4\%\\ 0.024\end{tabular}} & \begin{tabular}[c]{@{}l@{}}89.8\%\\ 0.094\end{tabular} \\ \hline
% 0.6 & \textbf{\begin{tabular}[c]{@{}l@{}}85.8\%\\ 0.211\end{tabular}} & \begin{tabular}[c]{@{}l@{}}82.8\%\\ 0.147\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}90.8\%\\ 0.160\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}90.6\%\\ 0.117\end{tabular}} \\ \hline
% 0.8 & \begin{tabular}[c]{@{}l@{}}84.2\%\\ 0.268\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}87.0\%\\ 0.113\end{tabular}} & \begin{tabular}[c]{@{}l@{}}88.4\%\\ 0.231\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}89.8\%\\ 0.158\end{tabular}} \\ \hline
% 0.9 & \begin{tabular}[c]{@{}l@{}}81.0\%\\ 0.367\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}86.8\%\\ 0.130\end{tabular}} & \begin{tabular}[c]{@{}l@{}}83.2\%\\ 0.336\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}91.0\%\\ 0.141\end{tabular}} \\ \hline
% 1.0 & \begin{tabular}[c]{@{}l@{}}61.4\%\\ 0.769\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}79.8\%\\ 0.239\end{tabular}} & \begin{tabular}[c]{@{}l@{}}58.8\%\\ 0.840\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}87.6\%\\ 0.233\end{tabular}} \\ \hline
% \end{tabular}%
% }
% \caption{Accuracy and resulting correlation between introduced feature and prediction for e-SNLI under different spurious cues and initial correlations between target variable and spurious feature}
% \label{tab: n-finetune-bias-strength}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllll}
% \hline
% Spurious cues, fine tuning n size & ComVE Standard & ComVE Explain & SBIC Standard & SBIC Explain \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present\\ Tense, n=1k\end{tabular} & \begin{tabular}[c]{@{}l@{}}92.4\%\\ 0.053\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}92.8\%\\ -0.004\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.241\end{tabular}} & \begin{tabular}[c]{@{}l@{}}77.4\%\\ 0.166\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present\\ Tense, n=4k\end{tabular} & \begin{tabular}[c]{@{}l@{}}81.6\%\\ 0.316\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}94.8\%\\ 0.021\end{tabular}} & \begin{tabular}[c]{@{}l@{}}65.4\%\\ 0.387\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}77.0\%\\ -0.001\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length, n=1k\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}91.4\%,\\ 0.134\end{tabular}} & \begin{tabular}[c]{@{}l@{}}89.4\%,\\ 0.108\end{tabular} & \begin{tabular}[c]{@{}l@{}}48.2\%\\ 0.772\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}51.6\%\\ 0.721\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length, n=4k\end{tabular} & \begin{tabular}[c]{@{}l@{}}83.2\%\\ 0.245\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}89.0\%\\ 0.109\end{tabular}} & \begin{tabular}[c]{@{}l@{}}50.4\%\\ 0.770\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}53.4\%\\ 0.670\end{tabular}} \\ \hline
% \end{tabular}%
% }
% \caption{Accuracy and resulting correlation between introduced feature and prediction for after increasing examples from 1k to 4k}
% \label{tab: n-increase experiments}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% Spurious Cues & CREAK Standard & CREAK Bootstrap & CREAK Explain \\ \hline
% \begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular} & \begin{tabular}[c]{@{}l@{}}60.4\%\\ 0.847\end{tabular} & \begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.045\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.325\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Embedding\\ Cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}74.6\%\\ 0.305\end{tabular} & \begin{tabular}[c]{@{}l@{}}73.0\%\\ 0.429\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.2\%\\ 0.146\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Present\\ Tense\end{tabular} & \begin{tabular}[c]{@{}l@{}}69.2\%\\ 0.563\end{tabular} & \begin{tabular}[c]{@{}l@{}}77.2\%\\ 0.167\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}78.6\%\\ 0.288\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Plural\\ Noun\end{tabular} & \begin{tabular}[c]{@{}l@{}}72.2\%\\ 0.445\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}80.8\%\\ 0.129\end{tabular}} & \begin{tabular}[c]{@{}l@{}}77.2\%\\ 0.170\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Accuracy and resulting correlation between introduced feature and prediction for CREAK dataset, including model generated explanations}
% \label{tab: CREAK explanation bootstrap}
% \end{table*}


\begin{table*}[t]
\begin{tabular}{p{2cm}p{3cm}p{4cm}p{5cm}}
\hline
 & Standard finetuned model & Standard prompting on standard finetuned model & Explanation-based prompting on standard finetuned model \\ \hline
Sentence Length & \begin{tabular}[c]{@{}l@{}}69.8\%\\ 0.467\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}78.4\% ($\uparrow$ 8.6\%)\\ 0.109 ($\downarrow$ 0.358)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}72.4\% ($\uparrow$ 2.6\%)\\ 0.148 ($\downarrow$ 0.319)\end{tabular} \\ \hline
Present Tense & \begin{tabular}[c]{@{}l@{}}76.0\%\\ 0.336\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}86\% ($\uparrow$ 10.0\%)\\ 0.039 ($\downarrow$ 0.297)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}83.6\% ($\uparrow$ 7.6\%)\\ 0.085 ($\downarrow$ 0.251)\end{tabular} \\ \hline
Embedding Cluster & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.595\end{tabular} & \begin{tabular}[c]{@{}l@{}}71.2\% ($\uparrow$ 0.6\%)\\ 0.532 ($\downarrow$ 0.063)\end{tabular} & \begin{tabular}[c]{@{}l@{}}62.8\% ($\downarrow$ 7.8\%)\\ 0.691 ($\uparrow$ 0.096)\end{tabular} \\ \hline
Plural Noun & \begin{tabular}[c]{@{}l@{}}69.0\%\\ 0.578\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}83.6\% ($\uparrow$ 14.6\%)\\ 0.219 ($\downarrow$ 0.359)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}78.6\% ($\uparrow$ 9.6\%)\\ 0.304 ($\downarrow$ 0.274)\end{tabular} \\ \hline
\end{tabular}
\caption{Standard few-shot prompting vs. explanation-based few-shot prompting on standard finetuned model with e-SNLI dataset}
\label{tab: few-shot-over-finetuned experiments}
\end{table*}


\subsection{Results on other models}

\minisection{GPT3-Ada}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllll}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c}{ComVE} & \multicolumn{2}{c}{CREAK} & \multicolumn{2}{c}{E-SNLI} & \multicolumn{2}{c}{SBIC} \\ \cline{2-9} 
 & Standard & Explain & Standard & Explain & Standard & Explain & Standard & Explain \\ \hline
No Cue & \textbf{79.2\%} & 52.4\% & \textbf{71.6}\% & 62.6\% & \textbf{88.0\%} & 76.4\% & \textbf{80.0\%} & 74.6\% \\ \hline
\begin{tabular}[c]{@{}l@{}}Sentence\\ Length\end{tabular} & \begin{tabular}[c]{@{}l@{}}44.8\%\\ 0.870\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}48.4\%\\ 0.778\end{tabular}} & \begin{tabular}[c]{@{}l@{}}53.0\%\\ 0.847\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}56.6\%\\ 0.590\end{tabular}} & \begin{tabular}[c]{@{}l@{}}60.4\%\\ 0.644\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}64.6\%\\ 0.531\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}53.6\%\\0.676\end{tabular}} & \begin{tabular}[c]{@{}l@{}}49.6\%\\ 0.712\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Present\\ Tense\end{tabular} & \begin{tabular}[c]{@{}l@{}}53.2\%\\ 0.956\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}54.0\%\\ 0.948\end{tabular}} & \begin{tabular}[c]{@{}l@{}}55.2\%\\ 0.738\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}55.8\%\\ 0.573\end{tabular}} & \begin{tabular}[c]{@{}l@{}}67.4\%\\ 0.586\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}69.6\%\\ 0.408\end{tabular}} & \begin{tabular}[c]{@{}l@{}}70.6\%\\ 0.461\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}75.2\%\\ 0.258\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Embedding\\ Cluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}47.6\%\\ 0.858\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}48.4\%\\ 0.807\end{tabular}} & \begin{tabular}[c]{@{}l@{}}50.2\%\\ 0.751\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}51.8\%\\ 0.705\end{tabular}} & \begin{tabular}[c]{@{}l@{}}55.8\%\\ 0.876\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}58.0\%\\ 0.753\end{tabular}} & \begin{tabular}[c]{@{}l@{}}56.0\%\\ 0.447\end{tabular} & \begin{tabular}[c]{@{}l@{}}55.0\%\\ 0.428\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Plural\\ Noun\end{tabular} & \begin{tabular}[c]{@{}l@{}}51.8\%\\ 0.853\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}53.8\%\\ 0.774\end{tabular}} & \begin{tabular}[c]{@{}l@{}}53.0\%\\ 0.775\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}53.8\%\\ 0.484\end{tabular}} & \begin{tabular}[c]{@{}l@{}}52.6\%\\ 0.911\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}58.4\%\\ 0.702\end{tabular}} & \begin{tabular}[c]{@{}l@{}}70.8\%\\ 0.393\end{tabular} & \textbf{\begin{tabular}[c]{@{}l@{}}71.8\%\\ 0.234\end{tabular}} \\ \hline
\end{tabular}%
}
\caption{Similar to Table 4, but run with OpenAI's smaller Ada model (2.7B Parameters)}
\label{tab: ada results}
\end{table*}
